Limits of Efficiency in Sequential Auctions

We study the efficiency of sequential first-price item auctions at (subgame perfect) equilibrium. This auction format has recently attracted much attention, with previous work establishing positive results for unit-demand valuations and negative results for submodular valuations. This leaves a large gap in our understanding between these valuation classes. In this work we resolve this gap on the negative side. In particular, we show that even in the very restricted case in which each bidder has either an additive valuation or a unit-demand valuation, there exist instances in which the inefficiency at equilibrium grows linearly with the minimum of the number of items and the number of bidders. Moreover, these inefficient equilibria persist even under iterated elimination of weakly dominated strategies. Our main result implies linear inefficiency for many natural settings, including auctions with gross substitute valuations, capacitated valuations, budget-additive valuations, and additive valuations with hard budget constraints on the payments. Another implication is that the inefficiency in sequential auctions is driven by the maximum number of items contained in any player's optimal set, and this is tight. For capacitated valuations, our results imply a lower bound that equals the maximum capacity of any bidder, which is tight following the upper-bound technique established by Paes Leme et al. \cite{PaesLeme2012}.

==> mpxerr.tex <==
\gdef\mpxshipout{\shipout\hbox\bgroup
  \setbox0=\hbox\bgroup}
\gdef\stopmpxshipout{\egroup  \dimen0=\ht0 \advance\dimen0\dp0
  \dimen1=\ht0 \dimen2=\dp0
  \setbox0=\hbox\bgroup
    \box0
    \ifnum\dimen0>0 \vrule width1sp height\dimen1 depth\dimen2 
    \else \vrule width1sp height1sp depth0sp\relax
    \fi\egroup
  \ht0=0pt \dp0=0pt \box0 \egroup}
\mpxshipout% line 8 C:/Users/vasilis/Dropbox/Research/MSR2012/Sequential Auctions/game-tree.mp
I_2%
\stopmpxshipout
\mpxshipout% line 12 C:/Users/vasilis/Dropbox/Research/MSR2012/Sequential Auctions/game-tree.mp
I_1^1%
\stopmpxshipout
\mpxshipout% line 16 C:/Users/vasilis/Dropbox/Research/MSR2012/Sequential Auctions/game-tree.mp
I_1^2%
\stopmpxshipout
\mpxshipout% line 26 C:/Users/vasilis/Dropbox/Research/MSR2012/Sequential Auctions/game-tree.mp
Y^1%
\stopmpxshipout
\mpxshipout% line 31 C:/Users/vasilis/Dropbox/Research/MSR2012/Sequential Auctions/game-tree.mp
Y^2%
\stopmpxshipout
\mpxshipout% line 36 C:/Users/vasilis/Dropbox/Research/MSR2012/Sequential Auctions/game-tree.mp
Y^3%
\stopmpxshipout
\mpxshipout% line 41 C:/Users/vasilis/Dropbox/Research/MSR2012/Sequential Auctions/game-tree.mp
Y^4%
\stopmpxshipout
\mpxshipout% line 46 C:/Users/vasilis/Dropbox/Research/MSR2012/Sequential Auctions/game-tree.mp
Y^5%
\stopmpxshipout
\mpxshipout% line 57 C:/Users/vasilis/Dropbox/Research/MSR2012/Sequential Auctions/game-tree.mp
{$p_2$ wins}%
\stopmpxshipout
\mpxshipout% line 59 C:/Users/vasilis/Dropbox/Research/MSR2012/Sequential Auctions/game-tree.mp
{$p_2$ loses}%
\stopmpxshipout
\mpxshipout% line 61 C:/Users/vasilis/Dropbox/Research/MSR2012/Sequential Auctions/game-tree.mp
{$p_2$ wins}%
\stopmpxshipout
\mpxshipout% line 62 C:/Users/vasilis/Dropbox/Research/MSR2012/Sequential Auctions/game-tree.mp
{$p_1$ wins}%
\stopmpxshipout
\mpxshipout% line 64 C:/Users/vasilis/Dropbox/Research/MSR2012/Sequential Auctions/game-tree.mp
{$p_2$ wins}%
\stopmpxshipout
\mpxshipout% line 65 C:/Users/vasilis/Dropbox/Research/MSR2012/Sequential Auctions/game-tree.mp
{$p_1$ wins}%
\stopmpxshipout
\mpxshipout% line 66 C:/Users/vasilis/Dropbox/Research/MSR2012/Sequential Auctions/game-tree.mp
{$a$ or $b$ wins}%
\stopmpxshipout
\mpxshipout% line 68 C:/Users/vasilis/Dropbox/Research/MSR2012/Sequential Auctions/game-tree.mp
{---}%
\stopmpxshipout
\mpxshipout% line 69 C:/Users/vasilis/Dropbox/Research/MSR2012/Sequential Auctions/game-tree.mp
{$u_a = 0$}%
\stopmpxshipout
\mpxshipout% line 70 C:/Users/vasilis/Dropbox/Research/MSR2012/Sequential Auctions/game-tree.mp
{$u_b = \alpha-\epsilon$}%
\stopmpxshipout
\mpxshipout% line 71 C:/Users/vasilis/Dropbox/Research/MSR2012/Sequential Auctions/game-tree.mp
{$u_c = \epsilon$}%
\stopmpxshipout
\mpxshipout% line 72 C:/Users/vasilis/Dropbox/Research/MSR2012/Sequential Auctions/game-tree.mp
{$u_d = 0$}%
\stopmpxshipout
\mpxshipout% line 74 C:/Users/vasilis/Dropbox/Research/MSR2012/Sequential Auctions/game-tree.mp
{$c$ wins}%
\stopmpxshipout
\mpxshipout% line 75 C:/Users/vasilis/Dropbox/Research/MSR2012/Sequential Auctions/game-tree.mp
{$u_a = 0$}%
\stopmpxshipout
\mpxshipout% line 76 C:/Users/vasilis/Dropbox/Research/MSR2012/Sequential Auctions/game-tree.mp
{$u_b = \alpha-\epsilon$}%
\stopmpxshipout
\mpxshipout% line 77 C:/Users/vasilis/Dropbox/Research/MSR2012/Sequential Auctions/game-tree.mp
{$u_c = \alpha$}%
\stopmpxshipout
\mpxshipout% line 78 C:/Users/vasilis/Dropbox/Research/MSR2012/Sequential Auctions/game-tree.mp
{$u_d = \alpha-\epsilon$}%
\stopmpxshipout
\mpxshipout% line 80 C:/Users/vasilis/Dropbox/Research/MSR2012/Sequential Auctions/game-tree.mp
{$b$ wins}%
\stopmpxshipout
\mpxshipout% line 81 C:/Users/vasilis/Dropbox/Research/MSR2012/Sequential Auctions/game-tree.mp
{$u_a = \epsilon$}%
\stopmpxshipout
\mpxshipout% line 82 C:/Users/vasilis/Dropbox/Research/MSR2012/Sequential Auctions/game-tree.mp
{$u_b = \alpha$}%
\stopmpxshipout
\mpxshipout% line 83 C:/Users/vasilis/Dropbox/Research/MSR2012/Sequential Auctions/game-tree.mp
{$u_c = \epsilon$}%
\stopmpxshipout
\mpxshipout% line 84 C:/Users/vasilis/Dropbox/Research/MSR2012/Sequential Auctions/game-tree.mp
{$u_d = 0$}%
\stopmpxshipout
\mpxshipout% line 86 C:/Users/vasilis/Dropbox/Research/MSR2012/Sequential Auctions/game-tree.mp
{$b$ or $c$ wins}%
\stopmpxshipout
\mpxshipout% line 87 C:/Users/vasilis/Dropbox/Research/MSR2012/Sequential Auctions/game-tree.mp
{$u_a = \epsilon$}%
\stopmpxshipout
\mpxshipout% line 88 C:/Users/vasilis/Dropbox/Research/MSR2012/Sequential Auctions/game-tree.mp
{$u_b = 0$}%
\stopmpxshipout
\mpxshipout% line 89 C:/Users/vasilis/Dropbox/Research/MSR2012/Sequential Auctions/game-tree.mp
{$u_c = 0$}%
\stopmpxshipout
\mpxshipout% line 90 C:/Users/vasilis/Dropbox/Research/MSR2012/Sequential Auctions/game-tree.mp
{$u_d = \alpha-\epsilon$}%
\stopmpxshipout
\end{document}

